A Dichotomy on the Complexity of Consistent Query Answering for Atoms with Simple Keys

We study the problem of consistent query answering under primary key violations. In this setting, the relations in a database violate the key constraints and we are interested in maximal subsets of the database that satisfy the constraints, which we call repairs. For a boolean query Q, the problem CERTAINTY(Q) asks whether every such repair satisfies the query or not; the problem is known to be always in coNP for conjunctive queries. However, there are queries for which it can be solved in polynomial time. It has been conjectured that there exists a dichotomy on the complexity of CERTAINTY(Q) for conjunctive queries: it is either in PTIME or coNP-complete. In this paper, we prove that the conjecture is indeed true for the case of conjunctive queries without self-joins, where each atom has as a key either a single attribute (simple key) or all attributes of the atom.

==> acyclic.tex <==
\section{Dichotomy for DAGs}
\label{sec:acyclic}

In this section, we prove a dichotomy for \cqa{$Q$} into P and coNP-complete in the case where the graph $G[Q]$ is a directed acyclic graph (DAG). We will assume w.l.o.g. that for every inconsistent edge $(x,y)$, there is no directed path $x \leadsto y$ (by applying \autoref{cor:double_path}).

We will first present a necessary condition to prove coNP-hardness, which we call {\em unsplittability}. Then, we will proceed to show that the condition is also sufficient, hence completing the dichotomy.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The coNP-complete Case}
\label{subsec:hardness}

For an inconsistent edge $e_R = (u_R, v_R)$, define 
%
\begin{align*}
fd(R) = \setof{u \in V(G)}{\exists \text{ path } u_R \leadsto v \text{ in } G -\{e_R\}}
\end{align*}
%
In other words, $fd(R)$ contains all the nodes that are reached from $u_R$ through a directed path that does not use edge $e_R$.

\begin{definition}
A pair of inconsistent edges $e_R, e_S$ is {\em unsplittable} if $u_R \neq u_S$ and there exists an undirected path $v_R \leftrightarrow u_S$ that does not contain any node from $fd(R)$ and similarly an undirected path $v_S \leftrightarrow u_R$ that does not contain any node from $fd(S)$. Otherwise, the pair is {\em splittable}.
\end{definition}

\begin{theorem}
\label{thm:hardness}
If $G[Q]$ contains an unsplittable pair of edges, \cqa{$Q$} is coNP-complete.
\end{theorem} 
 
This subsection will focus on the proof of \autoref{thm:hardness} in detail. To simplify our hardness construction, we can assume w.l.o.g. that any edge which is not $e_R$ or $e_S$ is consistent. Thus, from now on, $G$ contains only two inconsistent edges. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The PTIME Algorithm}

Suppose that every pair of inconsistent edges in the graph $G[Q]$ is splittable. We will then show that one can solve \cqa{$Q$} in polynomial time. Our algorithm is based on the notion of an {\em isolated set}. 

\begin{definition} [Isolated Set]
A set of inconsistent edges $E^{iso}$ is {\em isolated} if there exists a set of nodes $V^{iso}$ such that (a) if $R \in E^{iso}$ and $v \in V^{iso}$, there exists a consistent path $u_R \rightarrow v$ and (b) if an inconsistent edge $S \notin E^{iso}$, any path that connects some $R \in E^{iso}$ with $S$ has a node in $V^{iso}$. 
\end{definition}

In this case, we say that $V^{iso}$ {\em isolates} $E^{iso}$ from the rest of the inconsistent nodes. 

\begin{example}
Consider the graph $G[Q_a]$ in \autoref{fig:q_graph}. The graph contains an isolated set $E^{iso} = \{R_2, R_3\}$, where $V^{iso} = \{y,z\}$. Indeed, notice that condition (a) is satisfied, since there is a consistent path from $u$ (the source of both edges) to $y$ and $z$. As for condition (b), notice that node $y$ cuts completely both edges $R_2, R_3$ from the only other inconsistent edge $R_1$. Finally, notice that $V^{iso}$ could be only node $y$ as well.
\end{example}

In the remaining subsection, we will first show that if every pair of inconsistent edges is splittable, an isolated set always exists. Then, we will prove that the existence of such a set implies that the problem can be split into smaller independent problems that we can solve recursively. 

\paragraph{Finding an Isolated Set}

For a node $u$, let $Reach(u) = \setof{v}{u \rightarrow v}$, \ie the set of nodes that are reachable from $u$ through a consistent path. Define the node set $V^i = \{u_1, \dots, u_{\ell}\}$ to be the set of the source nodes of the inconsistent edges. Let us say that a node $u_i \in V^i$ is {\em terminal} if there is no consistent path $u_i \rightarrow u_j$ for some $u_j \in V^i$.

For an inconsistent edge $e_R = (u_R, v_R)$, let $split(R)$ be the set of inconsistent edges that are cut by $u_R$: in other words, $S \in split(R)$ if every path from $v_R$ to $S$ is cut by some node in $Reach(u_R)$. 

Our first goal is to find a pair of inconsistent edges $e_R,e_S$ such that the nodes $u_R, u_S$ are nicely behaved. More precisely, we show the following lemma.

\begin{lemma}
\label{lem:case_split}
For a DAG $G$ where every pair of inconsistent edges is splittable, exactly one of the following holds:
\begin{packed_enum}
\item There exist two edges $R,S$ s.t. $u_R, u_S$ are terminal nodes and either $S \in split(R)$ or $R \in split(S)$.
\item There exists a node $u \in V^i$ s.t. for any $u_i \in V^i$, there exists  a path $u_i \rightarrow u$.
\end{packed_enum}
\end{lemma}

\begin{proof}
We will first construct a graph $G^{s}$ as follows: for every node in $V^i$ introduce a node in $G^s$, and if there exists a consistent path $u_i \rightarrow u_j$, introduce a directed edge $(u_i, u_j)$. Observe that $G^s$ is a DAG, since $G$ is acyclic.  Hence, we can topologically order the nodes of $G^s$: assume w.l.o.g. that the order is $u_1, \dots, u_{\ell}$. Consider the topologically last node $u_{\ell}$, which by construction has no outgoing edges in $G^s$. 

In order to prove the lemma, notice that (1) and (2) are exclusive events. Hence, we will assume that (2) does not hold, and then show that this implies (1). Since (2) does not hold, there exist some node $u_j, j <\ell$ such that $(u_j, u_{\ell}) \notin E(G^s)$: consider the topologically largest such node, $u_j$. Notice that $u_j$ has no outgoing edges in $G^s$ as well: indeed, if an edge $(u_j, u_k)$ exists, where $j<k$, then $u_k$ would have to connect to $u_{\ell}$, a contradiction, since then transitively $u_j$ would connect to $u_{\ell}$. The pair of nodes $u_j, u_{\ell}$ are then terminal. 

Hence, $G$ contains two terminal nodes $u_1, u_2$. If $u_1, u_2$ are sources of unique inconsistent edges $e_R, e_S$, we have completed the proof. Indeed, since $R,S$ are splittable, any path from $v_R$ to $S$ will contain a node $v$ from $fd(R)$. However, this means that there exists a path $u_R \leadsto v$ that does not go through $e_R$; hence the path is a consistent path $u_R \rightarrow v$ (since $u_R$ is terminal) and any such path is cut by $Reach(u_R)$. In this case, $S \in split(R)$ (we considered this outcome w.l.o.g.).  

However, node $u_1$ may have inconsistent edges to $t_1, \dots, t_m$ and node $u_2$ inconsistent edges to $s_1, \dots, s_k$. If $Reach(u_1)$ cuts every path from some $t_i$ to $u_2$, we are done: $(u_2, s_j)$ (for any $j$) will belong in $split((u_1, t_i))$. Otherwise, for every node $t_i$, there will be a path to $u_2$ that is not cut by $Reach(u_1)$. Among all these paths, take the one where, if we remove the forward directed path, the remaining is of minimum length. Let $t_i \leadsto v$ the forward part and $v \leftrightarrow u_2$ the remaining. By our minimality assumption, $u_1$ cannot cut this path after $v$ by a path that goes through some $t_j$. However, it cannot be cut before $v$ or at $v$, since then we would have a double path, which would imply that $u_1$ cuts the path through $Reach(u_1)$. Hence, for the edge $e_1 = (u_1,t_i)$, $t_i$ has a path to $u_2$ not cut by $fd(e_1)$. We can make a symmetrical argument for $u_2$; however, now there can be no edge $e_2 = (u_2, s_j)$ such that $s_j$ has a path to $u_1$ not cut by $fd(e_2)$ (since then $e_1, e_2$ would be unsplittable). Consequently, we can always find the well-behaved pair of nodes that satisfies condition (1).  
\end{proof}

The lemma is used to show the following theorem, which proves the existence of an isolated set.

\begin{theorem}
\label{thm:isolated}
If every pair of inconsistent edges is splittable, there always exists an isolated set.
\end{theorem}

\begin{proof}
We start by applying \autoref{lem:case_split} to graph $G$. If condition (2) holds, then there exists a node $u$ such that for every inconsistent edge $S$, $u_S$ has a consistent path to $u$. Then, $E^i$ is an isolated set where $V^{iso} = u$ and condition (b) holds vacuously. The more interesting case is when condition (1) holds: then, we can find two edges $R, S$ such that $u_R, u_S$ are terminal nodes. Since $R,S$ are splittable, we can assume w.l.o.g. that $S \in split(R)$, \ie $u_R$ cuts every path from $v_R$ to the edge $S$. We distinguish two cases. 

In the first case, $split(R) = E^i \setminus \{R\}$. This implies that $u_R$ cuts every path from $v_R$ to any other edge: hence, $\{R\}$ is an isolated set, where $V^{iso} = Reach(u_R)$.  

In the second case, $split(R) \subset E^i \setminus \{R\}$; thus, there exists an inconsistent edge $T \notin split(R)$, where $T \neq R$. If for any such $T$ there exists a consistent path $u_T \rightarrow u_R$, then the set $E^i \setminus split(R)$ is isolated again, where $V^{iso} = Reach(u_R)$. Indeed, notice that every source node of an edge has a path to $u_R$ (and hence to $Reach(u_R)$). Additionally, if $v_T$ has a path to some edge $U$ in $split(R)$, this path can not be cut by $u_R$; but then, we will have a path from $v_R$ to $U$, a contradiction.


Otherwise, there is no consistent path from $u_T$ to $u_R$. Recall that $T \notin split(R)$  implies that there exists a path from $v_R$ to $T$ that is not cut by $u_R$. However, $u_T$ is not necessarily a terminal node. However, if $u_T$ is not a terminal node, $u_T$ has a consistent path to some $u_{T'}$ such that $u_{T'}$ is terminal and source of the inconsistent edge $T'$. We need to show that $T' \notin split(R)$. Indeed, by our initial assumptions, there exists a path $v_R \leftrightarrow u_T$ that is not cut by $u_R$. Moreover, there exists a consistent path $u_T  \rightarrow  u_{T'}$: no node of this path can be cut by $u_R$, since in this case there would be a consistent path $u_R \rightarrow u_{T'}$, which would contradict the fact that $u_{T'}$ is a terminal node.

The final step is to show that $split(T') \supset split(R)$. This concludes the proof, since we have found a new inconsistent edge where the source node is terminal and its split size has increased by at least one. Then, we can reapply our previous argument to either find the isolated set or find an edge with an even bigger split size. Since the split size is bounded, at some point the process will end and we will have found the isolated set.

To show our claim, we first prove that $split(R) \subseteq split(T')$. Indeed, consider any edge $S \in split(R)$ and assume that $S \notin split(T')$. This implies that there exists a path $p$ from $v_{T'}$ to $S$ not cut by $u_{T'}$. Now, $p$ must be cut somewhere by $u_R$, otherwise there would be a path  $v_R \leftrightarrow u_{T'} \leftrightarrow S$ not cut by $u_R$, contradicting our assumption that $S \in split(R)$. However, this implies that there exists another path $p'$ that connects $u_R$ to $v_{T'}$ not cut by $u_{T'}$, which would mean that $R,T'$ are not splittable, a contradiction. In order to finish our claim, note that $R \in split(T')$ (otherwise $R,T'$ would be splittable), whereas $R \notin split(R)$.
\end{proof}

\paragraph{Problem Splitting}
By applying \autoref{thm:isolated}, we can find a set of inconsistent edges $E^{iso}$ that are isolated by a set of nodes $V^{iso}$. We next describe how to take advantage of the existence of such a structure.

Consider the smallest possible set $V^{iso}$ and let it be $V^{iso} = \{w_1, \dots, w_k\}$. Now, let a possible evaluation of the tuple $(w_1, \dots, w_k)$ to some $\mathbf{a} = (a_1, \dots, a_k)$. Since every source node of an edge in $E^{iso}$ has a consistent path to every node in $V^{iso}$, for each $R \in E^{iso}$, there exists a set of values $m_R(\mathbf{a}) \subseteq Dom_G(u_R)$ such that every such value maps to the tuple $\mathbf{a}$. The crucial observation is that, for $\mathbf{a} \neq \mathbf{a}'$, we must have that $m_R(\mathbf{a}) \cap m_R(\mathbf{a}') = \emptyset$. 
%Indeed, if not, there would be a value $a$ from $u_R$ that maps to two different values of some node in $V^{iso}$, a contradiction.  

Now, let $r(\mathbf{a})$ refer to the set of all frugal repairs that contain $\mathbf{a}$ in the answer. Let $G^{iso}$ be the induced graph that contains all nodes in $V^{iso}$, along with the nodes of the isolated edges and any node that, after having removed $V^{iso}$, is still connected to some edge in $E^{iso}$.  Consider a new instance of \cqa{}, where $G^{iso}$ is our graph and for each edge $R \in E^{iso}$, the relation is limited only to key-groups from $m_R(\mathbf{a})$. Let $I(\mathbf{a})$ be this sub-instance of the database.

If this new instance has no satisfying repair, we immediately have that $r(\mathbf{a}) = \emptyset$. Indeed, the choices for the other values of a $R \in E^{iso}$ or for edges not in $I$ cannot influence whether $\mathbf{a}$ will be in the answer or not. On the other hand, assume that every repair is satisfying. Then, \cqa{$Q$} will be oblivious to the choices we make in $I(\mathbf{a})$.

This implies the following recursive process. For each such $\mathbf{a}$, construct and solve the instance $I(\mathbf{a})$ for the graph $G^{iso}$. Let $A^{iso}= \setof{\mathbf{a}}{I(\mathbf{a}) \vDash G^{iso}}$. Then, replace in $G$ the subgraph $G^{iso}$ by an arbitrary new node $n^I$ that has edges to all nodes in $V^{iso}$. Moreover,  for $w_i \in V^{iso}$ the relation corresponding to the edge $S_i(n^I, w_i)$ will contain a tuple $S_i(\mathbf{a}, a_i)$ for every $\mathbf{a} \in A^{iso}$. Let $G'$ be the newly constructed instance. 

\begin{example}
Continuing our example on $G[Q_a]$, $G^{iso}$ will be the graph $G[Q_a]$ without the edge $R_1(\ux,y)$. We can solve any instance on $G^{iso}$ in a straightforward way, since we can make a choice for each value of $u$ independently. Then, $G'$ will be the graph: $R_1(\ux,y), S_y(\underline{n^I}, y)$. Since $S_y$ is a consistent edge, $G'$ contains only one inconsistent edge and can also be solved in the same straightforward way. Thus, we can compute \cqa{$Q_a$} in PTIME. 
\end{example}


To show that the recursion is valid, we have to show that $G^{iso}$ and $G'$ are strictly easier subproblems and also that the splittability condition remains intact for the subproblems. Indeed:

\begin{proof}
We first show that both $G^{iso}, G'$ are of smaller size. Clearly, $G'$ contains at least one less inconsistent edge than $G$. The base case where $G'$ contains exactly one inconsistent edge can be easily solved, since each choice of the inconsistent edge is independent of the others. As for $G^{iso}$, the only issue is when $G^{iso} = G$. But in this case, following from our construction, there exists a source node $u_S$ of an inconsistent edge $S$ such that the source of every other inconsistent edge in $G^{iso}$ has a consistent path to $u_S$. Then, each $a \in Dom_{G}(I)$ creates an independent repair subproblem $S(a)$. However, in $S(a)$ we can fix each choice of $S$ and solve the problem for each such fixing (since there are polynomially many). This reduces the number of inconsistent repairs in the subgraph by 1, thus making it strictly easier.

Finally, we show that the splittability condition remains intact for $G^{iso}$ and $G'$. First, consider $G^{iso}$. The only violation of the condition may happen when a path used to connect two edges $e_R,e_S$ and it goes outside of $G^{iso}$. But then the path must go through $V^{iso}$, hence both $u_R,u_S$ will still cut it. As for $G'$, consider a path $p$ that was cut by some node $u_R$ in at some node $v$ in $G^{iso}$. Since the directed path from $u_R$ to $v$ goes through $V^{iso}$, $v \in V^{iso}$. Hence, the path $p$ will be also cut by $u_R$ in $G'$. 
\end{proof}

Notice also that the recursion depth depends only on the size of the query, whereas the processing at each step is FO-expressible.

\begin{theorem}
\label{thm:ptime}
If every pair of inconsistent edges is splittable, \cqa{Q} can be computed in PTIME and it is also FO-expressible.
\end{theorem}





